Beam Search: Faster and Monotonic

Beam search is a popular satisficing approach to heuristic search problems that allows one to trade increased computation time for lower solution cost by increasing the beam width parameter. We make two contributions to the study of beam search. First, we show how to make beam search monotonic; that is, we provide a new variant that guarantees non-increasing solution cost as the beam width is increased. This makes setting the beam parameter much easier. Second, we show how using distance-to-go estimates can allow beam search to find better solutions more quickly in domains with non-uniform costs. Together, these results improve the practical effectiveness of beam search.

==> dead.tex <==
\begin{observation}
\label{obs:sameselection}
For each beam slot $c$, if the node which would be selected to fill that slot has an $f$-value greater than the current incumbent solution's, either its children would not have been selected to fill that slot in nextBeam or there would be no node available to fill that slot in nextBeam with $f$-values less than the incumbent solution's, because the node's children cannot have $f$-values lower than the parent's.
\end{observation}



\begin{lemma}
\label{lemma:identicallevels}
In Algorithm \ref{alg:monobeam} with width greater than $c$, the set of nodes selected for nextBeam slots 1 through $c$ at each level (indicated by executions of the loop beginning at line \ref{lin:stop}) will be identical to the nodes selected for nextBeam slots 1 through $c$ at that level in a search with width $c$.
\end{lemma}
\begin{proof} By induction on level.
This is trivially true at the first level, where the only node is the node for the start state and it is always inserted at slot 1.

At any level $n$, if the nodes selected for nextBeam slots 1 through $c$ at level $n-1$ are identical to the nodes selected for nextBeam slots 1 through $c$ at level $n-1$ by a search with width $c$, then the nodes selected for slots 1 through $c$ at level $n$ will be identical to the nodes selected for nextBeam slots 1 through $c$ at level $n$ by a search with width $c$. Note that the nodes selected for nextBeam at level $n-1$ will be the nodes on beam at level $n$. We know by Lemma \ref{lemma:slotselection} that the nodes selected at slots 1 through $c$ will be identical to those selected by a search with width $c$ at level $n$ because the contents of beam (passed down from level $n-1$) are identical.
\end{proof}



\begin{lemma}
\label{lemma:pruningsafe}
In Algorithms~\ref{alg:monobeam} and~\ref{alg:pruning} with an admissible heuristic, beam width greater than $k$, and an incumbent solution found at some slot greater than $k$, at all levels (indicated by executions of the loop beginning at line \ref{lin:stop}) we will select for nextBeam slots 1 through $k$ exactly those nodes selected in a search with width $k$ that could lead to a solution with cost less than the incumbent solution's cost.
\end{lemma}
\begin{proof} By induction on level.
This is true at the level where the incumbent solution is found, because we know from Observation \ref{obs:nogoodremoved} that we will not remove any nodes which could lead to a better solution. We also know that at this level no new nodes will be selected that were not selected by a search of width $k$, based on Observation \ref{obs:nonewnodes}. So this level will contain only those nodes which would have been selected by a search of width $k$ which could lead to a solution with cost less than solutionCost.

If the nodes selected at level $n-1$ were exactly those nodes which would have been selected by a search of width s which could lead to a solution with cost less than solutionCost, then the nodes selected at level $n$ will be exactly those nodes which would have been selected by a search of width $k$ which could lead to a solution with cost less than solutionCost. We know by line \ref{lin:ftest} of Algorithm \ref{alg:pruning} and Observation \ref{obs:nogoodremoved} that we will remove all children from the previous beam's nodes which cannot lead to a solution with cost less than solutionCost, and only those nodes when building candidates. Observation \ref{obs:nonewnodes} indicates that there may be some empty slots in the beam, so there may be a smaller set of nodes on candidates to select from than at a search with width $n-1$. However, lines \ref{lin:pathmax} and \ref{lin:setpathmax} ensure that $f$-values are non-decreasing from parent to child. Any node which would have ranked more poorly than the children of a pruned node would, itself, be pruned. Therefore, the nodes selected for nextBeam at level $n$ will be exactly those nodes which would have been selected by a search of width $k$ which could lead to a solution with cost less than solutionCost.
\end{proof}



The table in Figure \ref{fig:percent-table} shows the likelihood of getting a better or equivalent solution from monobeam across all domains tested with widths 30, 100, 300, 1000, 3000, 10000, 30000, and 100000. In the unit tiles domain on this wider-ranging set of widths, monobeam's likelihood of finding a solution as good as or better than beam search rises. As seen in Figure \ref{fig:non-monotonic-plot}, monobeam often suffers most at the lowest beam widths, so this broader range of widths includes more cases where it has found (and stuck with) a better solution while beam search could be swinging up or down in terms of solution quality.

\begin{figure*}[t!]
\begin{center}
\begin{tabular}{ c |  c  c  c  c  c  c  c  c  c  c  c  }
 & tiles & tiles & tiles & tiles & tiles & 20pancake & 20pancake & 50pancake & 70pancake & 20bw & 20bwdp\\
 & unit & heavy & sqrt & reverse & inverse & unit & heavy & unit & unit & unit & unit\\
\hline
mono dominates & 48 & 40 & 32 & 34 & 43 & 53 & 63 & 76 & 63 & 29 & 11\\
non-mono dominates & 51 & 59 & 67 & 66 & 56 & 46 & 36 & 23 & 36 & 70 & 88\\
monobead fails & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\
bead fails & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\
\end{tabular}
\end{center}
\caption{Percent of cases where each algorithm dominates or fails at the beam widths tested.}
\label{fig:percent-table}
\end{figure*}






 A beam search with width $k+1$ may expand $\alpha$ in slot $k+1$ at a shallower depth and for lower or equal cost than the search with width $k$ encountered it, and it may be added to our closed list. However, it is possible that the goal under $\alpha$ might not be found in the search with width $k+1$ because it was competing against a different set of nodes for selection than when $\alpha$ was encountered in the search with width $k$. Then when $\alpha$ is encountered again at a lower beam slot, it would be discarded as a duplicate. The solution under $\alpha$ would not be found. It is possible that no better solution will be found in slot $k+1$ and we have lost access to the solution found by a search of width $k$, causing us to fail to meet the guarantee of monotonicity.



%This is expected behavior, as the limitations enforced to ensure monotonicity cause those algorithms to have poorer performance, but that the stability of montonic behavior combined with the larger beam widths allows them to find and consistently return good quality solutions.




\subsection{Refilling Empty Beam Slots}

When nodes can have no children (for example, dead ends) or when pruning from duplicate elimination or a candidate solution causes no children to be kept from a node, there may be times at which \emph{candidates} is empty at line \ref{lin:candidatesnotempty} in Algorithm \ref{alg:monobeam} before the full beam has been processed. If all slots below the current one are also empty, those slots would stay empty for the remainder of the search. For example, if slot 1 in our beam empties at one level of the search, we will not be able to expand a node from slot 1 to fill it ever again. However, immediately after the first slot $s$ to produce (non-pruned) children is filled, we can use nodes still on candidates to fill those empty lower slots. We call this approach \textbf{monobeam-refill} and provide pseudocode for it in Algorithm \ref{alg:refill}. While the search order for monobeam-refill will differ from the search order of monobeam, this refilling approach can be done while preserving monotonicity. If we selected nodes to refill empty slots from any slot higher than $s$ (such as filling from what is left on candidates at the end of selecting for slots $s$ through $k$) we would risk having a different search order in slots $s$ and lower at different beam widths, because the set of nodes left on candidates at the end of beam selection will differ for different beam widths.\fix{W found this confusing} Refilling can be combined with duplicate detection by inserting the code from Algorithm \ref{alg:dedup} at lines \ref{refilldedup1} and \ref{refilldedup2} of Algorithm \ref{alg:refill} instead of inserting the duplicate removal code directly into Algorithm \ref{alg:monobeam}.

\begin{algorithm}[t!]
%\DontPrintSemicolon
\Begin{
\If{all slots below c were left empty}{
\For{i from c through 0}{
\If{candidates is nonempty \label{refilldedup1}}{
nextBeam[i] $\leftarrow \min f$-value node from candidates\;
remove nextBeam[c] from candidates\;
}
}
}
\Else{
\If{candidates is nonempty \label{refilldedup2}}{
nextBeam[c] $\leftarrow \min f$-value node from candidates\;
remove nextBeam[c] from candidates\;
}
}
}
\caption{Refilling empty beam slots, to replace lines \ref{lin:candidatesnotempty} through \ref{lin:removefromcandidates} of Algorithm \ref{alg:monobeam}}\label{alg:refill}
\end{algorithm}



\begin{theorem}
\label{refilling}
Algorithms \ref{alg:monobeam} and \ref{alg:refill} with an admissible heuristic and beam width $k+1$ will always return a solution with cost lower or equal to the cost of the best solution found by the same algorithm with beam width $k$, for all $k \geq 1$.
\end{theorem}
\begin{proof}
If no slots in the search with width $k+1$ empty, then none will be refilled. Search will be the same as monobeam without refilling and by Theorem \ref{theo:monotonicity} the theorem holds trivially.

\fromS{Need to rework this to be in line with the other proofs.}

\end{proof}










In unit cost domains, after we have found a goal, later levels of search would only return worse solutions and we can return the first goal we find from any beam slot.  In non-unit cost domains, however, it is possible that a lower cost solution may lie at a later level of the search. It is therefore possible that a higher beam slot may lead to a solution earlier than lower beam slots, but with a worse cost.




On the other hand, assume that all slots below a given slot s $\leq$ k become empty at some level of the search. Either those slots would have emptied out in a search with width k or they were emptied based on pruning using a candidate solution from slot k+1. If the slots would have emptied in a search with width k, then no solutions can be lost based on refilling them, because those slots had no more nodes available to search and this same action of refilling would have been taken by a search of width k. If the slots emptied due to solution-based pruning, then no solution with lower cost than the candidate used for pruning could have been found in those slots during a search with width k. \fromS{What about cuckoo nodes being introduced which cause nodes from slots s through k to be pushed off the beam?} \fix{good point - what if we consider shifting the beam `to the right'?}




\begin{figure*}[tp!]
\incfig{plots/mono/tiles/averages-strict-unit} % fix this to include d-based
\hspace*{-15pt}
\incfig{plots/d-based/tiles/averages-strict-heavy}
\hspace*{-15pt}
\incfig{plots/d-based/tiles/averages-strict-sqrt}

\incfig{plots/d-based/tiles/averages-strict-reverse}
\hspace*{-15pt}
\incfig{plots/d-based/tiles/averages-strict-inverse}
\hspace*{-15pt}
\incfig{plots/mono/20pancake/averages-strict-unit}

\incfig{plots/d-based/20pancake/averages-strict-heavy} % fix this to include d-based
\hspace*{-15pt}
\incfig{plots/mono/20bw/averages-strict-unit}
\hspace*{-15pt}
\incfig{plots/mono/20bwdp/averages-strict-unit}

 % there will be two more pancake plots (50pancake and 70pancake) and a correlation plot
 % ############ these are currently just placeholders #########
\incfig{plots/d-based/20pancake/averages-strict-heavy}
\hspace*{-15pt}
\incfig{plots/mono/20bw/averages-strict-unit}
\hspace*{-15pt}
\incfig{plots/mono/20bwdp/averages-strict-unit}

\caption{Great results!}
\label{fig:plots}
\end{figure*}





Consider a base case of a solution found in slot $1$ within a monobeam search with beam width k>1. No duplicate pruning will occur of nodes from slot $1$ based on the nodes searched in any slot $>$ 1 because line \ref{lin:widthtest} in Algorithm \ref{alg:dedup} disallows this. Therefore, no node along the path to a solution found in slot $1$ will be pruned away. Furthermore, no space will be introduced for additional cuckoo nodes to be selected for the beam other than what was explored in a search of width 1 because line \ref{lin:widthtest} in Algorithm \ref{alg:dedup} disallows eliminating any duplicate based on nodes found in slots $>$ 1. Therefore, no node along a path to the solution found by a monobeam search of width 1 is able to be pushed off the beam based on duplicate elimination. Thus, the solution in slot 1 will still be found so long as it is better than the solutions found in slots $>$ 1.

Consider a solution found in a slot s between 1 and k within a monobeam search with beam width k $>$ 1. As above, no node along a path to the solution found at slot s can be eliminated or pushed off the beam because of the restriction in line \ref{lin:widthtest} in Algorithm \ref{alg:dedup}. Because duplicate elimination would be performed by the same algorithm run with width s, the duplicate elimination done in slot s based on nodes explored in slots $<$ s will be the same as what was done in a width s search. Therefore, the same solution that was found in slot s will still be found, if it is better than solutions found at any slot $>$ s and the theorem holds.




If at slot c-1 candidates contained only a subset of the children of nodes in beam from 1 to slot c-1, then at slot c candidates contains only those nodes already on candidates and children of beam[c] added at line \ref{lin:addtocandidates}. There may be nodes removed at line \ref{lin:removefromcandidates}, but no other nodes will be added aside from children of the node at beam[c]. Therefore, by induction candidates for newBeam[c] are always a subset of the children of nodes in slots 1 to c of beam.




\begin{theorem}
\label{monotonicity}
A monobeam search with beam width $k+1$ will always return a solution with cost lower or equal to the cost of the solution it would have returned if it had been run with beam width $k$, for all $k \geq 1$.
\end{theorem}
\begin{proof}
At the beginning of search, the start node is expanded from beam slot 1 at depth 0. At every subsequent depth $d>1$, only nodes from slots $1$ through $k$ at depth $d-1$ have been expanded, if they exist.  When nodes are selected to fill slot $k$ at depth $d$, \emph{candidates} contains only the children of those nodes. The nodes selected for slots $1$ through $k$ at $d$ will therefore depend only on slots $1$ through $k$ at $d-1$ regardless of whether additional beam slots exist or not.  The only influence that higher slots can have on lower ones is indirect, through pruning.

There are three cases for the pruning mechanism when at least one solution has been found.  
\begin{itemize}
\item \label{mono-better-found} First, a solution may be found in slot $k+1$ with cost lower than the solution returned by a search with beam width $k$. Any candidate solution will be used for pruning away nodes at lower slots until the search terminates, at which time it will be returned. Because it has a lower cost than the solution found by a search with beam width $k$, the theorem holds. The pruning will change the search order at the lower slots, but in this case we have a candidate solution already which is better than the one found in the lower beam slots, and therefore the theorem holds.
\item \label{mono-worse-found} Second, a solution may be found in slot $k+1$ with greater cost than the one found in a search with width $k$. The search will use this solution's $g$ value to prune away only nodes with $f$ values greater than or equal to that solution, and all nodes in slots $1$ through $k$ with potential to generate a solution with cost lower than the solution found in slot $k+1$ will not be pruned and any lower cost solution from slots $1$ through $k$ will still be found and returned. We know that any node pruned has an $f$ value greater than the currently known solution, so it could not generate a solution better than the current one. If the node which would have been selected to fill a given slot $s \leq k$ is pruned, this means that all nodes available in {\em candidates} were pruned because the node selected has the minimum $f$ value. So that slot will remain empty at this level and no nodes can be expanded from that slot which would not have been expanded by a search with beam width $k$. At the next level, slot $s$ may be filled by nodes generated from slots $1$ through $s-1$, but these nodes would have $f$ values less than the nodes which would have been generated by the node which would have occupied slot $s$ in a search with width $k$, or they would be pruned away. Any nodes which are later used to fill slot $s$ must be the ones which would have been expanded in a search with beam width $k$. Therefore, all nodes which would have been expanded by a search with beam width $k$ and could lead to a better solution than the one found at slot $k+1$ will be expanded. The better solution will be found and returned instead of the solution found at slot $k+1$.
\item \label{mono-none-found} Third, and finally, if no solution is found in slot $k+1$, then no pruning occurs and the solution found in slots $1$ through $k$ will be returned, and the theorem holds.
\end{itemize}
\end{proof}

---------------------------------------------------------------
\fix{introduce PHC?}  To provide a point of reference for our assessment of the price of monotonicity, we will also consider an algorithm that we call parallel hill climbing (PHC), with pseudocode given in Algorithm \ref{alg:phc}.  In this scheme, once the beam is full, each slot in the next beam is filled by the most promising child of the corresponding slot in the previous beam.  Unlike in monobeam, the children of previous slots are not candidates.  Thus, PHC is even more restricted than monobeam.

\fromS{I can't tell whether the intent is to show results for PHC or just discuss the concept. If we're going to show results, we should include duplicate checking in the pseudocode and discuss how this makes it non-monotonic.}

\begin{algorithm}[t!]
%\DontPrintSemicolon
%\KwData{start,width}
\Begin{
solutionCost $\leftarrow \infty$\;
beam[1] $\leftarrow$ start\;
\While {at least one slot in the beam has a node and no solution found}{
nextBeam $\leftarrow [ ] $\;
\For{each beam slot c from 1 to width}{
candidates $\leftarrow \emptyset$\;
\If {beam[c] is a node}{
\For{each child of beam[c]}{
\If {child is a goal}{
\If{$f$(child) $<$ solutionCost}{
store as solution\;
solutionCost $\leftarrow f$(child)\;
}
}
\Else{
add child to candidates\;
}
}
\If {candidates is nonempty}{
nextBeam[c] $\leftarrow$ $\min f$-value node from candidates\;
}
}
}
}
beam $\leftarrow$ nextBeam\;
}
return solution\;
}
\caption{PHC(start,width)}\label{alg:phc}
\end{algorithm}
---------------------------------------------------------------



old versions of algorithm pseudocode:

\dofig
{\bncode
{\bf MonoBeam(start, width)} \\
01. beam[1] $\leftarrow$ start \\
02. while at least one slot in the beam has a node \\
03. \> candidates $\leftarrow \emptyset$, nextBeam $\leftarrow [ ] $ \\
04. \> for each beam slot c from 1 to width \\
05. \> \> if beam[c] is a node \\
06. \> \> \> for each child of beam[c] \\
07. \> \> \> \> if f(child) $<$ f(solution) \\
08. \> \> \> \> \> if child is a goal \\
09. \> \> \> \> \> \> store as solution \\
10. \> \> \> \> \> else add child to candidates \\
11. \> \> if candidates is nonempty \\
12. \> \> \> nextBeam[c] $\leftarrow \min f$-value node from candidates \\
13. \> \> \> remove nextBeam[c] from candidates \\
14. \> beam $\leftarrow$ nextBeam \\
15. return solution
\ecode}{Pseudocode for monotonic beam search.}{fig:monobeam}


\dofig
{\bnncode
{\bf Dedup(node)} \\
01. if node's state is in closed list \\
02. \> add node to closed \\
03. \> add node to candidates \\
04. else \\
05. \> dup = closed entry for node's state \\
06. \> if dup.width $\leq$ node.width and dup.g $\leq$ node.g \\
07. \> \> reject node \\
08. \> else \\
09. \> \> update closed entry to node \\
10. \> \> add node to candidates
\ecode}{Pseudocode for handling possible duplicates in monotonic beam search.}{fig:dedup}


\dofig
{\bnncode
{\bf MonoBeamRefill(start, width)} \\
01. beam[0] $\leftarrow$ start \\
02. while at least one slot in the beam has a node \\
03. \> candidates $\leftarrow \emptyset$, nextBeam $\leftarrow [ ] $ \\
04. \> for each beam slot c from 1 to width \\
05. \> \> if beam[c] is a node \\
06. \> \> \> for each child of beam[c] \\
07. \> \> \> \> if f(child) $<$ f(solution) \\
08. \> \> \> \> \> if child is a goal \\
09. \> \> \> \> \> \> store as solution \\
10. \> \> \> \> \> else add child to candidates \\
11. \> \> if all slots below c were left empty \\
12. \> \> \> for i from c through 0 \\
13. \> \> \> \> if candidates is nonempty \\
14. \> \> \> \> \> nextBeam[i] $\leftarrow \min f$-value node from candidates \\
15. \> \> else if candidates is nonempty \\
16. \> \> \> nextBeam[c] $\leftarrow \min f$-value node from candidates \\
17. \> beam $\leftarrow$ nextBeam \\
18. return solution
\ecode}{Pseudocode for monotonic beam search with refilling of empty beam slots.}{fig:refill}





\begin{tikzpicture}[-, sibling distance=1cm]
 
    \node[main node]{A}
    child {
    node[main node][label=above:{h=1}]{B}
        child {
            node[main node][label=above:{h=1}]{E}
            child {
                node[main node][label=above:{h=1}]{J}
                child {
                    node[font=\sffamily\Large]{$\hdots$} edge from parent[draw=none]
                    child {
                        node[font=\sffamily\Large]{$\hdots$}  edge from parent[draw=none]
                        child {
                            node[font=\sffamily\Large]{$\hdots$}  edge from parent[draw=none]
                            child {
                                node[main node][font=\sffamily\Huge]{*}
                            }
                        }
                    }
                }
            }
        }
    }
    child[missing]{}
    child {
        node[main node][label=above:{h=2}]{C}
        child {
            node[main node][label=above:{h=4}]{F}
            child {
                node[main node][label=above:{h=6}]{K}
                child {
                    node[font=\sffamily\Large]{$\hdots$} edge from parent[draw=none]
                    child {
                        node[font=\sffamily\Large]{$\hdots$}  edge from parent[draw=none]
                        child {
                            node[font=\sffamily\Large]{$\hdots$}  edge from parent[draw=none]
                            child {
                                node[main node][font=\sffamily\Huge]{*}
                            }
                        }
                    }
                }
            }
        }
        child {
            node[main node][label=above:{h=4}]{G}
            child {
                node[main node][label=above:{h=6}]{L}
                child {
                    node[font=\sffamily\Large]{$\hdots$} edge from parent[draw=none]
                    child {
                        node[font=\sffamily\Large]{$\hdots$}  edge from parent[draw=none]
                        child {
                            node[font=\sffamily\Large]{$\hdots$}  edge from parent[draw=none]
                            child {
                                node[main node][font=\sffamily\Huge]{*}
                            }
                        }
                    }
                }
            }
        }
        child {
            node[bold node][label=above:{h=3}]{H}
            child {
                node[main node][label=above:{h=5}]{M}
                child {
                    node[font=\sffamily\Large]{$\hdots$} edge from parent[draw=none]
                    child {
                        node[font=\sffamily\Large]{$\hdots$}  edge from parent[draw=none]
                        child {
                            node[main node][font=\sffamily\Huge]{*}
                        }
                    }
                }
            }
        }
    }
    child[missing]{}
    child {
        node[bold node][label=above:{h=3}]{D}
        child[missing]{}
        child {
            node[main node][label=above:{h=5}]{I}
                child {
                    node[font=\sffamily\Large]{$\hdots$} edge from parent[draw=none]
                    child {
                        node[font=\sffamily\Large]{$\hdots$}  edge from parent[draw=none]
                        child {
                            node[main node][font=\sffamily\Huge]{*}
                        }
                    }
                }
        }
        child [grow=right] {
        node {g=1} edge from parent[draw=none]
        child [grow=down] {
        node {g=2} edge from parent[draw=none]
        child [grow=down] {
        node {g=3} edge from parent[draw=none]
        child [grow=down] {
        node[font=\sffamily\Huge]{$\hdots$} edge from parent[draw=none]
        child [grow=down] {
        node {g=7} edge from parent[draw=none]
        child [grow=down] {
        node {g=8} edge from parent[draw=none]
        child [grow=down] {
        node {g=9} edge from parent[draw=none]
        }
        }
        }
        }
        }
        }
        }
    }
    
 
\end{tikzpicture}

==> makefile <==
PAPER = main
OUTPUT = icaps-22

export BIBINPUTS=.:../BIBLIO

default:
	pdflatex $(PAPER).tex	
	bibtex --min-crossrefs=99 $(PAPER)
	pdflatex $(PAPER).tex	
	pdflatex $(PAPER).tex
	mv $(PAPER).pdf $(OUTPUT).pdf

tr: 
	pdflatex "\def\trflagdefined{}\input{$(PAPER).tex}" $(PAPER).tex	
	bibtex --min-crossrefs=99 $(PAPER)
	pdflatex "\def\trflagdefined{}\input{$(PAPER).tex}" $(PAPER).tex	
	pdflatex "\def\trflagdefined{}\input{$(PAPER).tex}" $(PAPER).tex

clean:
	rm -f *~ *.aux *.log *.blg *.bbl tmp.tex

